Learning Markov Chain in Unordered Dataset

The assumption that data samples are independently identically distributed is the backbone of many learning algorithms. Nevertheless, datasets often exhibit rich structure in practice, and we argue that there exist some unknown order within the data instances. In this technical report, we introduce OrderNet that can be used to extract the order of data instances in an unsupervised way. By assuming that the instances are sampled from a Markov chain, our goal is to learn the transitional operator of the underlying Markov chain, as well as the order by maximizing the generation probability under all possible data permutations. Specifically, we use neural network as a compact and soft lookup table to approximate the possibly huge, but discrete transition matrix. This strategy allows us to amortize the space complexity with a single model. Furthermore, this simple and compact representation also provides a short description to the dataset and generalizes to unseen instances as well. To ensure that the learned Markov chain is ergodic, we propose a greedy batch-wise permutation scheme that allows fast training. Empirically, we show that OrderNet is able to discover an order among data instances. We also extend the proposed OrderNet to one-shot recognition task and demonstrate favorable results.

==> intro.tex <==
\section{Introduction}
\label{sec:intro}
{

Recent advances in deep neural networks offer a great potential for both supervised learning, e.g., classification and regression~\citep{glorot2011domain,krizhevsky2012imagenet,xu2015show,finn2017deep} and unsupervised learning, e.g., dimension reduction and density estimation~\citep{}

. For instance, Convolutional Neural Networks (CNNs) \citep{krizhevsky2012imagenet} provided an automated way for learning image feature representations. Compared to hand-crafted features, such as SIFT and SURF, these hierarchical deep features demonstrate superior performance in recognition \citep{xu2015show,finn2017deep} and transfer learning \citep{glorot2011domain} problems.
Another example is {\em learning to learn} for automatic parameter estimation. \citet{andrychowicz2016learning} proposed to update model parameters without any pre-defined update rule, such as stochastic gradient descent (SGD) or ADAM \citep{kingma2014adam}. Surprisingly, this update-rule-free framework showed better performance and faster convergence on both object recognition and image style transformation tasks. 
In this paper, we investigate the following question: given an unordered dataset where instances may exhibit some  {\em implicit} order, can we find this order in an unsupervised fashion?

%Such order often exists even when we are dealing with data that is most naturally thought of as conisiting of  i.i.d. samples from a common, though complex distribution. For example, a dataset of 2D joint locations on the body of the same person in still photograps taken on different days would be well modeled by a 3D articulated  joint model that is projected onto a plane. However, although the i.i.d assumption is justified, as postures that person took on different days are likely unrelated, it is possible to arrange the data instances on an imaginary new timeline in such a way that the joints follow an aticulated motion, or set of motions going through all observed poses in a way that makes each pose highly predictable giving the previous ones. This arrangement will depend on the person, as a ballerina's poses will obey different implied dynamics than the poses of a tennis player, but joint ordering and inference of the pose evolution dynamics can lead to a strong model that explains the correlations among joints not in terms of the independen latent variables but in terms of the movement that binds the data points into a single sequence.  To put it differently, if we reshuffle the frames of a video sequence, the data now can be modeled by an i.i.d model, but reconstructing the order can lead to an alternative model, where transitions among the frames are simpler and/or easier to fit than are the links between the latent structure and the observation. The ballerina's dancing, if sampled very sparsly, can be thought of as a reshuffled video sequence that needs to be reordered so that a temporal model can generate it.This type of data can be captured in both ways, using i.i.d latent structure or data ordering, but the discovery of latent structure becomes exponentially harder as more an more causes of variability are added to the data while at the same time getting more and more obscured , e.g., if the data instances are silhouettes of people of different shapes and sizes. 

We argue that such order often exists even when dealing with the data that are naturally thought of as being i.i.d. sampled from a common, though complex, distribution. For example, let's consider a dataset consisting of the joint locations on the body of the same person taken on different days. The data i.i.d. assumption is justified since postures of a person took on different days are likely unrelated. However, we can arrange the data instances so that the joints follow an articulated motion or a set of motions in a way that makes each pose highly predictable given the previous one. 
Although this arrangement depends on the person as, for example,  ballerina's pose might obey different dynamics than the pose of a tennis player, the simultaneous inference on the pose dynamics can lead to a robust model that explains the correlations among joints. To put differently, if we reshuffle the frames of a video clip, the data can now be modeled by an i.i.d. model. Nevertheless, reconstructing the order leads to an alternative model where transitions between the frames are easier to fit. The ballerina's dancing, if sampled very sparsely, can be thought of as a reshuffled video sequence that needs to be reordered such that a temporal model can generate it.


\begin{figure*}[t!]
	\centering
	\includegraphics[width=0.9\textwidth]{./fig/illustration.pdf}
	%\vspace{-2mm}
	\caption{\small Illustration of the proposed Generative Markov Networks (\models). The data are assumed to be generated from a Markov chain, and \models learn the permutation and the transitional operator simultaneously. The figure illustrates that we first train \models for the data in green circles (without knowing the data order) to recover the data permutation. Then, we apply the trained transition operator to the data in blue circles (without knowing the data order) to infer data permutation.}
	\label{fig:illus}
\end{figure*}

Another example for discovering the order in an unsupervised manner is to study the evolution or dynamics of a system that cannot be easily recorded, such as the evolution of a galaxy. Usually, the process takes millions or billions of years; and it is impossible for a human to collect serial data. A model, capable of extracting the order, can potentially recover the evolution through a snapshot of thousands of data points (by collecting images from different galaxies at the same time), allowing us to better understand how the galaxy changes over time. 
Furthermore, consider modeling molecular or cellular data instances. These processes are often too fast to permit entire trajectories or too destructive to allow multiple sampling. On the other hand, our model can provide an alternative way to learn the dynamics of the biological system.

One naive and obvious way to find the order in a dataset is to perform sorting based on a predefined distance metric; e.g., the Euclidean distance between image pixel values. However, the distance metrics have to be predefined differently according to distinct types/characteristics of the datasets at hand. A proper distance metric for one domain may not be a good one for other domains. For instance, the $p-$distance is a good measure for DNA/RNA sequences \citep{nei2000molecular} while it does not characterize the semantic distances between images. We argue that the key component of the ordering problem lies in the discovery of proper distance metric automatically and adaptively.



To approach this problem, we model the data instances by treating them as if they were generated from a Markov chain. We propose to simultaneously train the transition operator and find the best order by a joint optimization over the parameter space as well as all possible permutations. We term our model Generative Markov Networks (\models). One of the key ideas in the design of \models is to use neural networks as a soft lookup table to approximate the possibly huge but discrete transition matrix. This strategy allows \models to amortize the space complexity using a unified model. Furthermore, due to the differentiable property of neural networks, the transitional operator of \models can also generalize on unseen but similar data instances. Besides, to ensure the Markov chain learned by \models is ergodic, we propose a greedy batch-wise permutation scheme that allows fast training. Fig. \ref{fig:illus} illustrates our proposed model.

We further extend our model to one-shot recognition tasks, where only one labeled data is given per category in the target domain. Most of the current work in this area focuses on learning a specific distance metric \citep{koch2015siamese,vinyals2016matching,snell2017prototypical} or category-separation metric \citep{ravi2016optimization,finn2017model} for the given data. During the inference phase, one would then compute either the smallest distance or highest class prediction score between the support and query instances. Alternatively, from a generative modeling perspective, we can first generate samples from the learned Markov chain, starting at each of the support instances, evaluate the query instance under generated samples, and assign the label with the highest log-likelihood probability. 
%fit the query instances into the Markov chain and decide the labels with the highest log-likelihood. 

Empirically, we demonstrate that \models are able to discover implicit orders among data instances while performing comparably with many of the current state-of-the-art methods on one-shot recognition tasks.



 
}


==> related.tex <==

\section{Related Works and Discussions}
\label{sec:rela}
{
The proposed Generative Markov Networks assumes a Markov chain data generation process, and one of the fundamental ideas is utilizing a deep neural network for amortizing the large state space in the transitional operator. In this Section, we provide brief discussions on related deep generative models. Since we have also applied \models into one-shot learning tasks, we will discuss the differences between our model and recent researches in one-shot learning.

{\bf Deep Generative Models:} Deep generative models can be categorized into two classes \citep{song2017nice} based on the sampling methods: {\em ancestral sampling} and {\em iterative sampling}. Instances of \emph{ancestral sampling} models are Variational Auto-encoders (VAEs) \citep{kingma2013auto}, Generative Adversarial Networks (GANs) \citep{goodfellow2014generative}, and their families. In the inference phase, these approaches generated one sample from the model by performing a single inference pass from latent variables to data. Lots of attention are attracted in supervised \citep{lin2017adversarial}, semi-supervised \citep{dai2017good}, and unsupervised \citep{hsu2017unsupervised} applications.

As a comparison, methods based on {\em iterative sampling} performed multiple and iterative passes through all the variables in the corresponding graphical models. Usually, these methods involved simulating a Markov chain in the entire state space, and they aimed at improving quality of generated samples by mixing the underlying chain. Recent works on this line of research included~\citep{salakhutdinov2007restricted,hinton2009deep,salakhutdinov2010efficient,bengio2013generalized,bengio2014deep,sohl2015deep,bordes2017learning,song2017nice}.

Our approach can be categorized as an {\em iterative sampling}-based model. However, it has three significant differences comparing to previous works.
First, existing works assumed training instances are i.i.d. sampled from the stationary distribution of a Markov chain. On the other hand, we assume the data are sequentially generated from a Markov in an unknown order. The order can be recovered by our proposed \model and thus help us understand the implicit data relationships.
Second, prior approaches were proposed based on the notion of denoising models. In other words, their goal was generating high-quality images; on the other hand, we aim at discovering an implicit order in the dataset. 
Third, to the best of our knowledge, all the existing works were implicit models in the sense that they only admitted efficient sampling schemes. In contrast, the proposed \model is an explicit model where besides an efficient sampling procedure, the model maintains a tractable likelihood function that can be computed efficiently. 

{\bf One-Shot Learning:} Here, we focus on deep one-shot learning models which could be divided into two categories: {\em nonparametric} and {\em parametric} approaches. The former aimed at either learning a similarity measurement between instance pairs \citep{koch2015siamese} or applying specific metric loss based on cosine distance \citep{vinyals2016matching}/ Euclidean distance \citep{snell2017prototypical}. Usually, these methods relied heavily upon human design. 

As a comparison, methods in the second category offered more generalities. Typically, this type of methods tackled the problem using a meta-learning framework to train the {\em parametric} classifiers. Precisely, they considered two levels of learning: the first stage is to update base learners' parameters and the second stage is to update parameters for the meta learner. Recent works \citep{ravi2016optimization,kaiser2017learning,finn2017model} belonged to this category. 

\models is an instance of the first category and has the following difference. Instead of designing a specific loss for one-shot learning purpose, we employ Markov chain data generation assumption and determine the label of query instance by fitting it into the simulated Markov chain from support instances. 
 %This generative nature significantly decreases the difficulty of training as we no longer rely on any designed metric. More details will be covered in Sec. \ref{sec:exp}.


	
}
